On the Role of Postconditions in Dynamic First-Order Epistemic Logic

Dynamic Epistemic Logic (DEL) is a logic that models information change in a multi-agent setting through the use of action models with pre- and post-conditions. In a recent work, DEL has been extended to first-order epistemic logic (DFOEL), with a proof that the resulting Epistemic Planning Problem is decidable, as long as action models pre- and post-conditions are non-modal and the first-order domain is finite. Our contribution highlights the role post-conditions have in DFOEL. We show that the Epistemic Planning Problem with possibly infinite first-order domains is undecidable if the non-modal event post-conditions may contain first-order quantifiers, while, on the contrary, the problem becomes decidable when event post-conditions are quantifier-free. The latter result is non-trivial and makes an extensive use of automatic structures.

==> macrossophie.tex <==

%%%% Macros raccourcis %%%%%

\newcommand{\mb}[1]{\mathbb{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}

\renewcommand{\phi}{\varphi}

\renewcommand{\epsilon}{\varepsilon}

\newcommand{\es}{\vspace{1\baselineskip}}
\newcommand{\ds}{\vspace{0.5\baselineskip}}

\newcommand{\pc}{\preccurlyeq}
\newcommand{\bin}{\texttt{bin}}


\newcommand{\ap}{\textsf{AP}}

\newcommand{\ag}{\textsf{Ag}}

\newcommand{\lel}{{\textsf{EL}}}


%\newcommand{\pre}{{\textsf{pre}}}
%\newcommand{\post}{{\textsf{post}}}
%\newcommand{\dom}{{\textsf{dom}}}
\newcommand{\dirset}{\setevents}%{{\mc{E}}}
\newcommand{\dirsetStwoS}{\{1,2\}}%{{\mc{E}}}
\newcommand{\tree}{\mc{T}}
\newcommand{\treearity}{n}

\newcommand{\depth}{{\textsf{depth}}}

\newcommand{\del}{{\textsf{DEL}}\xspace}

\newcommand{\el}{\textsf{el}}
%% ajout de Sophie
\newcommand{\VarSet}{\mathcal{V}}

%%
%%%% end macros raccourcis %%%%%


%% rajouté par Sophie
%\newcommand{\lang}{\ensuremath{\mathcal{L}}}
\newcommand{\logic}{\ensuremath{\mathcal{L}}}
\newcommand{\avalu}{\valuationc}    %valuation
%% transducers
\newcommand{\transd}{{\mathcal A}}
%\newcommand{\blank}{\perp}
%\newcommand{\pad}{\paddingsymbol}
\newcommand{\alphabet}{\Sigma}
\newcommand{\extalphabetconv}{\Sigma_{\pad}}
\newcommand{\extalphabet}{\Sigma_{\blank}}
\newcommand{\word}{u}
\newcommand{\wordb}{v}
\newcommand{\transddelta}{\transd_\Dom}
\newcommand{\transdepsilon}{\transd_\epsilon}
\newcommand{\transdi}[1][i]{\transd_{#1}}

%% automatic structures
\newcommand{\Dom}{D}
\newcommand{\elem}{d}
\newcommand{\rel}{R}
\newcommand{\func}{r}

\newcommand{\FOstruct}{{\mathcal S}}
\newcommand{\FOstructtuple}{\FOstruct = \langle \Dom, \rel_1 \dots \rel_p \rangle}
\newcommand{\FOtreetuple}{\langle \Dom, r,\suc_1, \dots, \suc_n, \rel_1, \dots, \rel_p \rangle}
\newcommand{\AS}{A}
\newcommand{\AStuple}{(\transddelta, \transdi[1], \ldots, \transdi[p])}
\newcommand{\ASpresent}{\AS=\AStuple}

\newcommand{\Chainstruct}{\mc{C}}
\newcommand{\Chain}{Ch}
\newcommand{\chain}{C}
\newcommand{\Chainstructtuple}[1][\Chain]{\Chainstruct = \langle \Dom, \rel_1 \dots \rel_p,#1 \rangle}

\newcommand{\decfunc}{\encfunc^{-1}}
\newcommand{\encfunc}{\texttt{\upshape enc}}

\newcommand{\langdelta}{L_{\Dom}}
\newcommand{\langepsilon}{L_{\epsilon}}
\newcommand{\langrel}[1][i]{L_{#1}}

\newcommand{\wordchain}{C}
%% regular automatic trees
\newcommand{\rootnode}{r}
\newcommand{\addresse}{\encfunc}
\newcommand{\suc}{S}
\newcommand{\FOtree}{{\mathcal T}}
\newcommand{\FOKtreetuple}{\FOtree = \langle \Dom, \rootnode, \suc_1, \ldots, \suc_n,\lknow{1} \dots \lknow{m},(p)_{p \in AP} \rangle}
\newcommand{\AT}{T}
\newcommand{\ATtuple}{\langle \transddelta, \transd_\rootnode, (\transdi')_{1 \leq i \leq  \treearity}, (\transdi)_{1 \leq i \leq  p} \rangle}
\newcommand{\ATpresent}{\AT=\ATtuple}


\newcommand{\foform}{\Psi}
%\newcommand{\Branch}{\Pi}
\newcommand{\branch}{\pi}
\newcommand{\Branches}{\textsf{Branches}}
\newcommand{\encoding}{\gamma}
\newcommand{\Tree}{\textsf{Tree}}

\newcommand{\mbranch}{\textsf{mbranch}}
\newcommand{\code}{\encfunc}%{\textsf{code}}
% logics
\newcommand{\valu}{\sigma}
\newcommand{\Varfo}{\Var_1}
\newcommand{\Varmso}{\Var_2}
\newcommand{\Sing}[1]{\textsf{Sing}(#1)}
\newcommand{\Singonly}{\textsf{Sing}}
\newcommand{\isBranchfrom}[2]{\textsf{pathfrom}[#1,#2]}
%\newcommand{\isBranchto}[2]{\textsf{pathto}[#1,#2]}
%\newcommand{\fromtoBranch}[3]{\textsf{pathfromto}[#1,#2,#3]}
\newcommand{\Inf}{\textsf{Inf}}
\newcommand{\U}{\text{\textsf{U}}}
\newcommand{\X}{\text{\textsf{X}}}
\newcommand{\E}{\text{\textsf{E}}}
\newcommand{\A}{\text{\textsf{A}}}
\newcommand{\F}{\text{\textsf{F}}}
\newcommand{\G}{\text{\textsf{G}}}

\newcommand{\mso}{{\textsf{MSO}}\xspace}
\newcommand{\cmso}{{\textsf{cMSO}}\xspace}
\newcommand{\chainmso}{{\textsf{chain-MSO}}\xspace}
\newcommand{\pmso}{{\textsf{path-MSO}}\xspace}
\newcommand{\logicCTLstar}{{\textsf{CTL$^*$}}\xspace}
\newcommand{\logicCTLstarK}{{\textsf{CTL$^*$K}}\xspace}
\newcommand{\cmsok}{{\textsf{cMSO}}\text{K}\xspace}
\newcommand{\fo}{\textsf{FO}\xspace}
\newcommand{\fow}{\textsf{FO}\text{$(\exists^\omega)$}}
\newcommand{\ltl}{\textsf{LTL}}
\newcommand{\ctl}{\textsf{CTL}}
\newcommand{\ctlk}{\text{\textsf{CTLK}}}
\newcommand{\ctls}{$\textsf{CTL}^*$}
\newcommand{\ctlsk}{\text{\textsf{CTL}$^*$K}}
\newcommand{\ectls}{\text{\textsf{ECTL}$^*$}\xspace}
\newcommand{\lmulin}{\text{\textsf{L}$^{\textsf{lin}}_{\mu}$}} % linear-time mu-calculus
\newcommand{\blmulin}{\text{B}\lmulin} % branching linear-time mu-calculus
\newcommand{\blmulink}{\text{B}\lmulin\text{K}} % branching linear-time mu-calculus
%\newcommand{\blmulink}{\text{\textsf{L}$^*${lin$_{\mu}$K}} % branching linear-time mu-calculus
  %\newcommand{\muc}{{\mu\textsf{CTL}}}
\newcommand{\muc}{\blmulin}
%% Buchi
\newcommand{\automaton}[1][]{{\mathcal A}_{#1}}
%\newcommand{\BautomatonChain}[1][m]{\mc{C}_{#1}}
\newcommand{\langautomaton}{L}
\newcommand{\codepair}[2]{\left(\substack{#1\\ #2}\right)}
\newcommand{\automatontransition}[1]{\stackrel{#1}{\rightarrow}}
% misc
\newcommand{\tr}{tr}
\newcommand{\trELtoFO}{\tau}
\newcommand{\setn}{\mb{N}}

\newcommand{\lettera}{\mathsf a}
\newcommand{\letterb}{\mathsf b}
\newcommand{\letterainteger}{\mathtt 0}
\newcommand{\letterbinteger}{\mathtt 1}
\newcommand{\pairvertical}[2]{\left(\substack{#1\\ #2}\right)}
\newcommand{\tripletvertical}[3]{\left(\substack{#1\\ #2\\ #3}\right)}

%%%%% again from AiML 2018
\newcommand{\relhiststar}{\relhist^*}
\newcommand{\trace}{h}
\newcommand{\history}{\trace}
\newcommand{\traceSet}{\mathcal H}
% \newcommand{\DELpres}[1][]{(\stateext[#1],\eventmodel_{#1})}
\newcommand{\DELpres}[1][]{(\stateext,\action_{#1})}
\NewDocumentCommand{\update}{O{}}{\modelM \otimes \eventmodel^{#1}}
\NewDocumentCommand{\DELstruct}{O{*}}{\modelM \eventmodel^{#1}}
% \newcommand{\DELstructPOINTED}[1][]{\stateext[#1] \eventmodel_{#1}^*}
\newcommand{\DELstructPOINTED}[1][]{\stateext \action_{#1}^*}
\newcommand{\DELstructfull}{\DELstruct=
	(\traceSet,\relhist, \relhiststar, \{\relM{\agent}\}_{\agent\in\agtset},\valuationfunction)}
\newcommand{\DELstructOnlyKnowledgeAndRelHistfull}{\DELstruct=
	(\traceSet,(\suc_\event)_{\event\in\dirset}, (\epistemicrelation{\agent})_{\agent\in\agtset},(\atom)_{\atom \in \atmset})}
        
 % \newcommand{\pointed}{\begin{tikzpicture}
 %         	\node[line width=0.4mm, draw=black, circle, inner sep=0.5mm, minimum height=1mm, minimum width=1mm] {};
 %         	\end{tikzpicture}}
 \newcommand{\pointed}{\begin{tikzpicture}
         	\node[line width=0.35mm, draw=black, circle, inner sep=0.4mm, minimum height=0.4mm, minimum width=0.5mm] {};
         	\end{tikzpicture}}        
%   \newcommand{\pointed}{\bullet}
        
\newcommand{\DELstructOnlyKnowledgeAndRelHistfullPOINTED}{\DELstructPOINTED=
	(\traceSet,(\suc_\event)_{\event\in\dirset}, (\epistemicrelation{\agent})_{\agent\in\agtset},(\atom)_{\atom \in \atmset},\pointed)}
        
\newcommand{\DELstructOnlyKnowledgefull}{\DELstruct=
	(\traceSet, \{\relM{\agent}\}_{\agent\in\agtset},\valuationfunction)}


\newcommand{\languageEpistemic}{\mathscr{L}_{EL}}

%% to be removed?
\newcommand{\exempleSpecificationTextOne}{invariantly, an intruder $\agent$ does not know the location of the piece of jewelry more than 3 consecutive steps}
\newcommand{\exempleSpecificationTextTwo}{all \fsmodiffinalversion{drones} know that the region is safe every 20 steps}
\newcommand{\exempleSpecificationTextThree}{\fsmodiffinalversion{with the current plan, the drone $\agent$ never knows the region is safe but every 10 steps, there is a(nother) plan to let the drone $\agent$ eventually know the region is safe}}


\newcommand{\paddingsymbol}{\scalebox{0.7}{\ensuremath{\square}}}

